Three Conjectures on Binary Channels for the Doubly Symmetric Binary Source

We settle three conjectures concerning a doubly symmetric binary source $(X,Y)$ with crossover $p$. Consider Markov chains $U - X - Y - V$ with $U,V$ binary, and let $\mathcal{A}$ be the set of rate triples $(I(U;V),I(U;X),I(Y;V))$ attainable with arbitrary binary channels $X\to U$, $Y\to V$, and $\mathcal{B}$ the subset attainable with binary symmetric channels. The averaged BSC conjecture, Conjecture 5.2 of Pichler, Piantanida and Matz (2022), asserts $\operatorname{conv}\mathcal{A}=\operatorname{conv}\mathcal{B}$. We prove this for every $p\in[0,1]$. Two conjectures of Dikshtein, Ordentlich and Shamai (2022) concern the double-sided information bottleneck at $p=0$, where $Y=X$ and the two channels see the same source: their Conjecture 1 identifies the exact maximum of $I(U;V)$ at prescribed rates $I(U;X)$ and $I(Y;V)$, and their Conjecture 2 the exact minimum. We prove both for binary $U,V$: the two extrema are attained by the same pair of Z/S-channels, in opposite orientation for the maximum and in the same orientation for the minimum. The proofs were found with substantial AI assistance, and all three theorems are formalised in Lean 4 with Mathlib, depending only on the standard axioms. The development is available at https://github.com/g-pichler/bsc-averaging . The proof of Conjecture 1 of Dikshtein, Ordentlich and Shamai (2022) contains three certified computations, a polynomial bound, an interval sweep and a polynomial positivity certificate, all of which are checked in Lean.

==> generated/facts.tex <==
% Generated by Paper/Facts.lean from the Lean development -- do not edit.
% Regenerate with `make facts` in paper1/.
\newcommand{\NCells}{88}
\newcommand{\CellRationals}{528}
\newcommand{\SweepLo}{0.45}
\newcommand{\SweepHi}{3}
\newcommand{\CellWidthMin}{0.002}
\newcommand{\CellWidthMax}{0.149}
\newcommand{\CellWidthMinGrid}{2}
\newcommand{\CellWidthMaxGrid}{149}
\newcommand{\CellWidthGridDen}{1000}
\newcommand{\SweepHalvings}{4}
\newcommand{\SweepTerms}{10}
\newcommand{\SweepGrid}{10^{9}}
\newcommand{\KronSlots}{371293}
\newcommand{\KronBase}{2^{64}}
\newcommand{\CertBideg}{(12,12)}
\newcommand{\CertMonomialsTotal}{41405}
\newcommand{\QDeg}{52}
\newcommand{\QTerms}{53}
\newcommand{\QFirstCoeffs}{q_0=\tfrac{4}{15},\quad q_1=-\tfrac{7}{1440},\quad q_2=\tfrac{979}{1440},\quad q_3=-\tfrac{175}{1728},\quad q_4=\tfrac{6821}{8640},\quad q_5=-\tfrac{32473}{103680}}
\newcommand{\QLastIndex}{52}
\newcommand{\QLastCoeff}{-\frac{282\,475\,249}{754\,598\,979\,313\,436\,528\,297\,902\,080\,000\,000\,000}}
\newcommand{\QHatZero}{0.2666}
\newcommand{\QTailStart}{21}
\newcommand{\QTableRows}{0 & $0.2666$ & 7 & $-0.4172$ & 14 & $-0.0197$ \\ 1 & $-0.0049$ & 8 & $0.0086$ & 15 & $-0.0150$ \\ 2 & $0.6798$ & 9 & $-0.3149$ & 16 & $-0.0051$ \\ 3 & $-0.1013$ & 10 & $-0.0846$ & 17 & $-0.0032$ \\ 4 & $0.7894$ & 11 & $-0.1566$ & 18 & $-0.0010$ \\ 5 & $-0.3133$ & 12 & $-0.0539$ & 19 & $-0.0006$ \\ 6 & $0.3723$ & 13 & $-0.0558$ & 20 & $-0.0002$ \\}
\newcommand{\QNegSum}{0.0191}
\newcommand{\LeanToolchain}{v4.32.2}

